Flexible-Latency DRAM: Understanding and Exploiting Latency Variation in Modern DRAM Chips

This article summarizes key results of our work on experimental characterization and analysis of latency variation and latency-reliability trade-offs in modern DRAM chips, which was published in SIGMETRICS 2016, and examines the work's significance and future potential. The goal of this work is to (i) experimentally characterize and understand the latency variation across cells within a DRAM chip for these three fundamental DRAM operations, and (ii) develop new mechanisms that exploit our understanding of the latency variation to reliably improve performance. To this end, we comprehensively characterize 240 DRAM chips from three major vendors, and make six major new observations about latency variation within DRAM. Notably, we find that (i) there is large latency variation across the cells for each of the three operations; (ii) variation characteristics exhibit significant spatial locality: slower cells are clustered in certain regions of a DRAM chip; and (iii) the three fundamental operations exhibit different reliability characteristics when the latency of each operation is reduced. Based on our observations, we propose Flexible-LatencY DRAM (FLY-DRAM), a mechanism that exploits latency variation across DRAM cells within a DRAM chip to improve system performance. The key idea of FLY-DRAM is to exploit the spatial locality of slower cells within DRAM, and access the faster DRAM regions with reduced latencies for the fundamental operations. Our evaluations show that FLY-DRAM improves the performance of a wide range of applications by 13.3%, 17.6%, and 19.5%, on average, for each of the three different vendors' real DRAM chips, in a simulated 8-core system.

==> sec/algos/readcl.tex <==
\floatname{algorithm}{Test}
%\captionsetup[algorithm]{labelsep=none}
%\renewcommand{\thealgorithm}{}

\begin{algorithm}

\begin{algorithmic}[1]
\algrenewcommand\algorithmicfunction{}
%\algrenewcommand\algorithmicindent{1.2em}
\algrenewcommand\algorithmicdo{}
\algrenewcommand\alglinenumber[1]{\footnotesize\texttt{#1}}
\algrenewcommand\algorithmicindent{1.2em}
\small

\Function{ReadOneCacheLine}{$\mathit{my\_tRCD}, \mathit{my\_tRP}, \mathit{bank},
\mathit{row}, \mathit{col}$}
\State {\tt ACT(}$\mathit{bank}, \mathit{row}${\tt )}
\State {\tt cmdDelay(}$\mathit{my\_tRCD}${\tt )} \Comment{Set activation latency
(\trcd)}
\State {\tt READ(}$\mathit{bank}, \mathit{row}, \mathit{col}${\tt )}
\State {\tt cmdDelay(}\tcl+\tbl{\tt )} \Comment{Wait for
read to finish}
\State {\tt PRE(}$\mathit{bank}${\tt )}
\State {\tt cmdDelay(}$\mathit{my\_tRP}${\tt )} \Comment{Set precharge latency
(\trp)}

\State {\tt readData()} \Comment{Send the read data from FPGA to PC}
%\State {\tt findErrors()}

\EndFunction
\end{algorithmic}

\caption{Read a cache line with specified timing parameters.}
\label{readcl}
\end{algorithm}


==> sec/algos/trcdlocal.tex <==
\floatname{algorithm}{Test}
%\captionsetup[algorithm]{labelsep=none}
%\renewcommand{\thealgorithm}{}

\begin{algorithm}[h]

\algnewcommand\algorithmicto{\textbf{to}}
\algrenewtext{For}[3]{\algorithmicfor\ #1 $\gets$ #2 \algorithmicto\ #3 \algorithmicdo}

\algrenewcommand\algorithmicfunction{}
\algrenewcommand\algorithmicdo{}
\algrenewcommand\algorithmicindent{1.2em}
\algrenewcommand\alglinenumber[1]{\footnotesize\texttt{#1}}
\small

\begin{algorithmic}[1]
%\Function{tRCDRowReadTest}{$\mathit{my\_tRCD}, \mathit{data}$}
\Function{ReadOneRow}{$\mathit{my\_tRCD}$, $\mathit{bank}, \mathit{row}$}

%\For{b}{1}{$\mathit{Bank}_{\mathit{MAX}}$}
%\For{r}{1}{$\mathit{Row}_{\mathit{MAX}}$}
%
%\State {\tt WriteOneRow(}$\mathit{b}, \mathit{r}, \mathit{data}${\tt)}
%\State {\tt ReadOneRow(}$\mathit{tRCD}, \mathit{tRP}, \mathit{b}, \mathit{r}${\tt)}
%\State {\tt assert findErrors() == 0} \Comment{Verify data}
%\State {\tt ReadOneRow(}$\mathit{\textbf{my\_tRCD}}, \mathit{tRP}, \mathit{b}, \mathit{r}${\tt)}
%\State {\tt findErrors()} \Comment{Count errors every cache line}

\State {\tt ACT(}$\mathit{bank}, \mathit{row}${\tt )}
\State {\tt cmdDelay(}$\mathit{\textbf{my\_tRCD}}${\tt )} \Comment{Set activation latency}

\For{c}{1}{$\mathit{Col}_{\mathit{MAX}}$}
\State {\tt READ(}$\mathit{bank}, \mathit{row}, \mathit{c}${\tt )} \Comment{Read
one cache line}
\State {\tt findErrors()} \Comment{Count errors in a cache line}
\EndFor
\State {\tt cmdDelay(}\tcl+ \tbl{\tt )}
\State {\tt PRE(}$\mathit{bank}${\tt )}
\State {\tt cmdDelay(}\trp{\tt )}

%\EndFor
%\EndFor

\EndFunction
\end{algorithmic}

\caption{Read one row with a specified \trcd value.}
\label{trcdlocal}
\end{algorithm}


==> sec/algos/trcdtest.tex <==
\floatname{algorithm}{Test}
%\captionsetup[algorithm]{labelsep=none}
%\renewcommand{\thealgorithm}{}

\begin{algorithm}[h]

\algnewcommand\algorithmicto{\textbf{to}}
\algrenewtext{For}[3]{\algorithmicfor\ #1 $\gets$ #2 \algorithmicto\ #3 \algorithmicdo}

\algrenewcommand\algorithmicfunction{}
\algrenewcommand\algorithmicdo{}
\algrenewcommand\algorithmicindent{1.2em}
\algrenewcommand\alglinenumber[1]{\footnotesize\texttt{#1}}
\small

\begin{algorithmic}[1]
\Function{tRCDColOrderTest}{$\mathit{my\_tRCD}, \mathit{data}$}

\For{b}{1}{$\mathit{Bank}_{\mathit{MAX}}$}
\For{c}{1}{$\mathit{Col}_{\mathit{MAX}}$} \Comment{Column first}
\For{r}{1}{$\mathit{Row}_{\mathit{MAX}}$}

\State {\tt WriteOneCacheLine(}$\mathit{b}, \mathit{r}, \mathit{c}, \mathit{data}${\tt)}
\State {\tt ReadOneCacheLine(}\trcd, \trp, $\mathit{b}, \mathit{r}, \mathit{c}${\tt)}
\State {\tt assert findErrors() == 0} \Comment{Verify data}
%\State {}
\State {\tt ReadOneCacheLine(}$\mathit{\textbf{my\_tRCD}}$, \trp, $
\mathit{b}, \mathit{r}, \mathit{c}${\tt)}
\State {\tt findErrors()} \Comment{Count errors in a cache line}

\EndFor
\EndFor
\EndFor

\EndFunction
\end{algorithmic}

\caption{Read each cache line with a specified \trcd value.}
\label{trcdtest}
\end{algorithm}
%\vspace{-0.05in}


==> sec/algos/trptest.tex <==
\floatname{algorithm}{Test}
%\captionsetup[algorithm]{labelsep=none}
%\renewcommand{\thealgorithm}{}

\begin{algorithm}[h]

\algnewcommand\algorithmicto{\textbf{to}}
\algrenewtext{For}[3]{\algorithmicfor\ #1 $\gets$ #2 \algorithmicto\ #3 \algorithmicdo}

\algrenewcommand\algorithmicfunction{}
\algrenewcommand\algorithmicdo{}
\algrenewcommand\algorithmicindent{1.2em}
\algrenewcommand\alglinenumber[1]{\footnotesize\texttt{#1}}
\small

\begin{algorithmic}[1]
\Function{tRPRowOrderTest}{$\mathit{my\_tRP}, \mathit{data}$}

\For{b}{1}{$\mathit{Bank}_{\mathit{MAX}}$}
%\For{c}{1}{$\mathit{Col}_{\mathit{MAX}}$} \Comment{Column first}
\For{r}{1}{$\mathit{Row}_{\mathit{MAX}}$} \Comment{Row order}

\State {\tt WriteOneRow(}$\mathit{b}, \mathit{r}, \mathit{data}${\tt)}
\State {\tt ReadOneRow(}\trcd, \trp, $\mathit{b}, \mathit{r} ${\tt)}
\State {\tt WriteOneRow(}$\mathit{b}, \mathit{r+1}, \mathit{data\_bar}${\tt)} \Comment{Inverted data}
\State {\tt ReadOneRow(}\trcd, \trp, $\mathit{b}, \mathit{r+1} ${\tt)}
\State {\tt assert findErrors() == 0} \Comment{Verify data, data\_bar}
%\State {}
\State {\tt ReadOneRow(}\trcd, $\mathit{\textbf{my\_tRP}},
\mathit{b}, \mathit{r}${\tt)}
\State {\tt findErrors()} \Comment{Count errors in row r}

\EndFor
%\EndFor
\EndFor

\EndFunction
\end{algorithmic}

\caption{Read each row with a specified \trp value.}
\label{trptest}
\end{algorithm}


==> sec/subplots/b1_rcd3_dimm_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{Bank0}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{Bank1}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank1_ecc0.pdf} }
    \subcaptionbox{Bank2}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank2_ecc0.pdf} }
    \subcaptionbox{Bank3}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank3_ecc0.pdf} }

    \subcaptionbox{Bank4}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank4_ecc0.pdf} }
    \subcaptionbox{Bank5}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank5_ecc0.pdf} }
    \subcaptionbox{Bank6}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank6_ecc0.pdf} }
    \subcaptionbox{Bank7}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank7_ecc0.pdf} }
    \caption{Error coverage overlapped from 12 experimental runs on DIMM A0 at \trcd=7.5ns at 20\celsius.}
    \label{fig:dimm_va_b1_rcd_20c}
\end{figure*}


==> sec/subplots/b1_rcd_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc1.pdf} }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc2.pdf} }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc3.pdf} }

    \caption{Effect of ECC on DIMM A0 at \trcd=7.5ns at 20\celsius.}
    \label{fig:b1_rcd_ecc_heatmap_20c}
\end{figure*}


==> sec/subplots/burst_rcd2_20c.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{Two DIMMs (A-M1).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd2.pdf}
    %}
    %%
    %\subcaptionbox{One DIMMs (B-M1).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd2.pdf}

    %}
    %%
    %\subcaptionbox{Six DIMMs (C-M0).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
    %}

    \subcaptionbox{A-M1}%[\linewidth]
    {
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }
    \subcaptionbox{B-M1}%[\linewidth]
    {
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }
    %
    \subcaptionbox{C-M0}[\linewidth]
    {
        %\includegraphics[scale=0.6]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }

    \caption{Breakdown of the number of error bits observed in each data
    beat of erroneous cache lines at \trcde5ns.}
    \label{fig:burst_rcd2_20c}
\end{figure}

%all_cr_m1_dimms_burst_rcd2.pdf
%all_hy_m1_dimms_burst_rcd2.pdf
%all_y_dimms_burst_rcd2.pdf

%\begin{figure*}[h]
%    \centering
%    \captionsetup[subfigure]{justification=centering}
%    \subcaptionbox{DIMM A0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/b1_all_patt_rcd2_20c.pdf}
%    }
%    %
%    \subcaptionbox{DIMM B0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_p6_all_att_rcd2.pdf}
%    }
%    %
%    \subcaptionbox{DIMM C0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_y22_all_patt_rcd2_20c.pdf}
%    }
%    %
%    \subcaptionbox{DIMM C5.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_g1_all_patt_rcd2_20c.pdf}
%    }
%
%    \caption{Breakdown on the number of error bits observed in data
%    bursts, which form a cache line, due to \trcd=5ns at 20\celsius.}
%    \label{fig:burst_rcd2_20c}
%\end{figure*}


==> sec/subplots/burst_rcd3_20c.tex <==
\begin{figure*}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{A-M1}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/b1_all_patt_rcd3_20c.pdf}
        \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd3.pdf}
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd2.pdf}
    }
    %
    \subcaptionbox{B-M1}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/p6_all_patt_rcd3.pdf}
        \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd3.pdf}
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd2.pdf}

    }
    %
    \subcaptionbox{C-M0}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/burst_dist_y22_all_patt_rcd3_20c.pdf}
        \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd3.pdf}
        %\includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
        %\includegraphics[scale=0.65]{plots/trcd/bursts/all_y_dimms_burst_rcd3.pdf}
    }

    \caption{Breakdown of the number of error bits observed in each data
    beat of erroneous cache lines \newt{at \trcde 7.5ns}.}
    \vspace{5pt}
    \label{fig:burst_rcd3_20c}
\end{figure*}

%all_cr_m1_dimms_burst_rcd2.pdf
%all_hy_m1_dimms_burst_rcd2.pdf
%all_y_dimms_burst_rcd2.pdf


==> sec/subplots/err_loc.tex <==
\begin{figure}[!h]
    \centering
		\captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Bank 0 of \dimm{0}{C}\label{fig:rcd_col_err}}[0.48\linewidth] {
        \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}
		}
    \subcaptionbox{Bank 0 of \dimm{3}{A}\label{fig:rcd_err_region}}[0.48\linewidth] {
        \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/y7_1125/ecc0/{filecnt_52_hist_128x16384_y7_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}
		}
        \caption{Probability of \newt{observing activation} errors.}
    \label{fig:err_loc}
\end{figure}


==> sec/subplots/memory.tex <==
\begin{figure}[h]
    \centering
		\captionsetup[subfigure]{justification=centering}
    \subcaptionbox{DRAM System\label{dram-organization}}[0.48\linewidth] {
        \includegraphics[scale=0.75]{plots/memory_system.pdf}
		}
    \subcaptionbox{DRAM Bank\label{bank-organization}}[0.48\linewidth] {
        \includegraphics[scale=0.75]{plots/dram_bank.pdf}
		}%
        \caption{DRAM \new{system organization}.}
    %\vspace{-5pt}
    \label{memory-organization}
\end{figure}


==> sec/subplots/p6_rcd_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc1.pdf} }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc2.pdf} }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc3.pdf} }

    \caption{Effect of ECC on DIMM B0 at \trcd=5ns at 20\celsius.}
    \label{fig:p6_rcd_ecc_heatmap_20c}
\end{figure*}


==> sec/subplots/rcd_ber_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.3\textwidth]
    {
        %\includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/crucial_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/crucial_model_patt0x0_ber.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.3\textwidth]
    {
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/hynix_model_patt0x0_ber.pdf}
    }
    %
    \subcaptionbox{Vendor C.}[0.3\textwidth]
    {
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/samsung_model_patt0x0_ber.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.225\textwidth]
    %{
    %    \includegraphics[width=0.225\linewidth]{plots/trcd/ber/ber_plots/samsung_g_ber_20c.pdf}
    %}

    %\caption{Bit error rates (BERs) of various DRAM DIMMs running at different \trcd parameters at 20\celsius.}
    \caption{Bit error rates (BERs) of DRAM DIMMs by their models running at different \trcd parameters.}
    \label{fig:rcd_ber_20c}
\end{figure*}


==> sec/subplots/rcd_ber_expand_model_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A and model A-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/crucial_ber_20c_model0.pdf}
    }
    %
    \subcaptionbox{Vendor B and model B-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/hynix_ber_20c_model0.pdf}
    }
    %
    \subcaptionbox{Vendor C and model C-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/samsung_ber_20c_model0.pdf}
    }

    \caption{Bit error rates (BERs) of various DIMMs with the same model running at different \trcd parameters.}
    \label{fig:rcd_ber_expand_model_20c}
\end{figure*}


==> sec/subplots/rcd_ber_pattern_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\dimm{0}{A}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/crucial_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/crucial_b1_ber_pattern_20c.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{B}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/hynix_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/hynix_p1_ber_pattern_20c.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{C}.\label{fig:pattern_vc}}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_y_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_y17_ber_pattern_20c.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_g_ber_pattern_20c.pdf}
    %}
    \caption{BERs due to four different data patterns as \trcd varies.}
    \label{fig:rcd_ber_pattern_20c}
\end{figure*}


==> sec/subplots/rcd_ber_temp.tex <==
\begin{figure*}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\dimm{0}{A}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/crucial_b1_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/crucialb1_temp_bars}.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{B}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/hynix_p1_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/hynixp1_temp_bars}.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{C}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/samsung_y17_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/samsungy17_temp_bars}.pdf}
    }
    %
    %\subcaptionbox{Vendor C, DIMM g1.}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_temp_plots/samsung_g1.pdf}
    %}

    \caption{BERs of various DRAM DIMMs operating under different temperatures.}
        %(average with 95\% confidence intervals).}
    \label{fig:rcd_ber_temp}
\end{figure*}


==> sec/subplots/rcd_ber_temp_vert.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\trcde7.5ns\label{fig:temp_rcd75}}[\linewidth]
    {
        \includegraphics[width=\linewidth]{{plots/temp_tRCD_75}.pdf}
    }

    \subcaptionbox{\trcde5ns\label{fig:temp_rcd50}}[\linewidth]
    {
        \includegraphics[width=\linewidth]{{plots/temp_tRCD_50}.pdf}
    }

    \caption{BERs of \new{three \newt{example}} DIMMs operating under different temperatures.}
        %(average with 95\% confidence intervals).}
    \label{fig:rcd_ber_temp}
\end{figure}


==> sec/subplots/rcd_error_breakdown_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_3_18.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/hynix_rcd_err_25C_p1_3_6.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch1.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/samsung_rcd_err_25C_y17_19_22.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch2.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/samsung_rcd_err_25C_g1_5_15.pdf}
    }

    \caption{Breakdown on the fraction of cache lines containing 0, 1, or $\ge$2
    erroneous bits in different DIMMs with varying tRCD values (ns) at 20\celsius.}
    \label{fig:rcd_error_breakdown_20c}
\end{figure*}


==> sec/subplots/rcd_error_breakdown_pattern_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A, DIMM b1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor B, DIMM p1.\label{fig:vb-p1-errbar-pattern-20c}}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/hynix_rcd_err_p1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch1, DIMM g1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_g1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch2, DIMM y17.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_y17_ff_00_cc_aa.pdf}
    }

    \caption{Different data patterns running at different
        tRCD parameters at 20\celsius.}
    \label{fig:rcd_error_breakdown_pattern_20c}
\end{figure*}


==> sec/subplots/rcd_error_breakdown_temp.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A, DIMM b1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor B, DIMM p1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/hynix_rcd_err_p1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor C, DIMM g1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_g1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor C, DIMM y17.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_y17_26_35_50_70C.pdf}
    }

    \caption{Breakdown on the fraction of cache lines containing 0, 1, or $\ge$2
        erroneous bits in different DIMMs with varying tRCD parameters operating
        under different temperatures.}
    \label{fig:rcd_error_breakdown_temp}
\end{figure*}


==> sec/subplots/rp_ber_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/crucial_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/crucial_trp_model_ber.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/hynix_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/hynix_trp_model_ber.pdf}
    }
    %
    \subcaptionbox{Vendor C.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/samsung_y_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/samsung_trp_model_ber.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.28\textwidth]
    %{
    %    \includegraphics[width=0.28\linewidth]{plots/trp/ber/samsung_g_ber_20c.pdf}
    %}

    \caption{Bit error rates (BERs) of various DRAM DIMMs by their models running at different \trp parameters.}
    \vspace{5pt}
    \label{fig:rp_ber_20c}
\end{figure*}


==> sec/subplots/scaling.tex <==
\begin{figure*}[!h]
    \centering
    %\captionsetup[subfigure]{justification=centering}
    \captionsetup[subfigure]{justification=justified}

    \subcaptionbox{\trcd xx.\vspace{0.1in}\label{fig:scaling_trcd}}%[\linewidth]
    {
        \includegraphics[scale=1]{plots/scaling_tRCD}
    }

    \subcaptionbox{\trp xx.\label{fig:scaling_trp}}%[\linewidth]
    {
        \includegraphics[scale=1]{plots/scaling_tRP}

    }

    \caption{xxxx.}
    \label{fig:scaling}
\end{figure*}


==> sec/subplots/timing_reduced.tex <==
\begin{figure}[t]
    \centering
    \captionsetup[figure]{justification=centering}
    \includegraphics[width=1.0\linewidth]{plots/timing_reduced}
    \caption{DRAM Operation with Reduced Timings}
    \label{fig:timing_reduced}
\end{figure}


==> sec/subplots/timing_standard.tex <==
\begin{figure}[t]
    \centering
    \captionsetup[figure]{justification=centering}
    \includegraphics[width=1.0\linewidth]{plots/timing_standard}
    \caption{Internal DRAM phases, DRAM command/data timelines, and timing
        parameters to read a cache line.}
    \label{fig:timing_standard}
    %\vspace{-0pt}
\end{figure}


==> sec/subplots/trp_err_loc.tex <==
\begin{figure}[!h]
    \centering
		\captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Bank 0 of \dimm{0}{C}\label{fig:rp_col_err_b0}}[0.38\linewidth] {
        \includegraphics[width=0.38\linewidth,height=1.2in]{plots/trp/heatmap/samsung_heatmap_trp/samsungy17/{filecnt_12_hist_128x16384_samsungy17_rp7.5ns_allpatts_20c_bank0}.pdf}
		}
    \subcaptionbox{Bank 7 of \dimm{0}{C}\label{fig:rp_col_err_b7}}[0.58\linewidth] {
        \includegraphics[width=0.58\linewidth,height=1.2in]{plots/trp/heatmap/samsung_heatmap_trp/samsungy17/{filecnt_12_hist_128x16384_samsungy17_rp7.5ns_allpatts_20c_bank7}.pdf}
		}
    %\subcaptionbox{Bank 0 of \dimm{3}{A}.\label{fig:rp_err_free_region}}[0.48\linewidth] {
    %    \includegraphics[width=0.48\linewidth]{plots/trp/heatmap/samsung_heatmap_trp/samsungy22/{filecnt_45_hist_128x16384_samsungy22_rp7.5ns_allpatts_20c_bank1}.pdf}
	%	}
    \caption{Probability of observing precharge errors.}
    \label{fig:trp_err_loc}
\end{figure}


==> sec/subplots/y17_rcd3_dimm_heatmap_20c.tex <==
\begin{figure}[!h]
    \centering

    \subcaptionbox{Bank0}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf} }
    \subcaptionbox{Bank1}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank1_ecc0}.pdf} }

    \subcaptionbox{Bank2}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank2_ecc0}.pdf} }
    \subcaptionbox{Bank3}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank3_ecc0}.pdf} }

    \subcaptionbox{Bank4}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank4_ecc0}.pdf} }
    \subcaptionbox{Bank5}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank5_ecc0}.pdf} }

    \subcaptionbox{Bank6}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank6_ecc0}.pdf} }
    \subcaptionbox{Bank7}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank7_ecc0}.pdf} }
    \caption{Probability of errors in \dimm{0}{C} at \trcd=7.5ns.}
    \label{fig:dimm_y17_rcd3}
\end{figure}


==> sec/subplots/y19_rp_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc0/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc0}.pdf}
    }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc1/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc1}.pdf}
    }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc2/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc2}.pdf}
    }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc3/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc3}.pdf}
    }

        \caption{Effect of ECC on \dimm{2}{C} at \trp=7.5ns at 20\celsius.}
    \label{fig:y19_rp_ecc_heatmap_20c}
\end{figure*}


==> sec/tables/scaling_dimms.tex <==
%%%%%%%%%%%%%%%%%
% Single Column
%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{0.9}
\begin{table}[h]
\small
  \centering
    \setlength{\tabcolsep}{1em}
    \begin{tabular}{ccccc}
        \toprule
        Tech.& Chip & DIMM & Assembly & DIMM \\
        Node & Density & Capacity & Year & Counts \\
        \midrule

        5xnm & 1Gb & 1GB & 2010    & 3 \\
        3xnm & 2Gb & 2GB & 2011-12 & 3$^{\dagger}$ \\
        29nm & 4Gb & 2GB & 2015    & 3 \\
        28nm & 4Gb & 2GB & 2015    & 3 \\

        \bottomrule
        % Footnote
        \multicolumn{5}{r}{
            $^\dagger$Two of the three DIMMs are \dimm{0}{B} and \dimm{1}{B}
            (\tabref{dimm_list}).
        }

    \end{tabular}
  \caption{Tested DIMMs from vendor B for the scaling study.}
  \label{tab:scaling_dimm_list}%
  %\vspace{-0.15in}
\end{table}


==> sec/tables/vldram_config.tex <==
%%%%%%%%%%%%%%%%%
% Single Column
%%%%%%%%%%%%%%%%%
\begin{table}[h]
    \renewcommand{\arraystretch}{1.2}
    \small
    \centering
    %\setlength{\tabcolsep}{.2em}
    \begin{tabular}{cccrrrr}
        \toprule
        \multirow{2}{*}{DIMM} &
        \multirow{2}{*}{Vendor} & \multirow{2}{*}{Model} &
        \multicolumn{2}{c}{\trcd Dist. (\%)}  & \multicolumn{2}{c}{\trp Dist. (\%)} \\
        \cmidrule(l{2pt}r{2pt}){4-5}
        \cmidrule(l{2pt}r{2pt}){6-7}
        Name & & & 7.5ns & 10ns & 7.5ns & 10ns\\
        \midrule

        \dimm{2}{A} & A & M1 & 93 & 7 & 74 & 26 \\
        \dimm{7}{B} & B & M1 & 12 & 88 & 13 & 87 \\
        \dimm{2}{C} & C & M0 & 99 & 1 & 99 & 1 \\

        \bottomrule
    \end{tabular}
    \caption{Distribution of cache lines under various \trcd and \trp values for three
    characterized DIMMs.}
    \label{tab:vldram_config}%
\end{table}

% crucial 2 M1
% hynix 7 M1
% samsung 2 M0

